A system-wide network reconstruction of gene regulation and metabolism in Escherichia coli

Genome-scale metabolic models have become a fundamental tool for examining metabolic principles. However, metabolism is not solely characterized by the underlying biochemical reactions and catalyzing enzymes, but also affected by regulatory events. Since the pioneering work of Covert and co-workers as well as Shlomi and co-workers it is debated, how regulation and metabolism synergistically characterize a coherent cellular state. The first approaches started from metabolic models which were extended by the regulation of the encoding genes of the catalyzing enzymes. By now, bioinformatics databases in principle allow addressing the challenge of integrating regulation and metabolism on a system-wide level. Collecting information from several databases we provide a network representation of the integrated gene regulatory and metabolic system for Escherichia coli, including major cellular processes, from metabolic processes via protein modification to a variety of regulatory events. Besides transcriptional regulation, we also take into account regulation of translation, enzyme activities and reactions. Our network model provides novel topological characterizations of system components based on their positions in the network. We show that network characteristics suggest a representation of the integrated system as three network domains (regulatory, metabolic and interface networks) instead of two. This new three-domain representation reveals the structural centrality of components with known high functional relevance. This integrated network can serve as a platform for understanding coherent cellular states as active subnetworks and to elucidate crossover effects between metabolism and gene regulation.

==> pgflibraryarrows.new.code.tex <==
% alternative * arrow
\pgfarrowsdeclare{* new}{* new}
{
  \ifdim\pgfgetarrowoptions{* new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=5.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=1.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{* new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \ifdim\pgfgetarrowoptions{* new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%  
    \pgfpathcircle{\pgfqpoint{-3\pgfutil@tempdima}{0pt}}{+4.5\pgfutil@tempdima}
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{* new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 2%
    \pgfpathcircle{\pgfqpoint{\pgfutil@tempdima}{0pt}}{\pgfutil@tempdima}
    \pgfusepathqfillstroke
  \fi
}

% alternative round bracket arrow
\pgfarrowsdeclare{( new}{) new}
{
  \ifdim\pgfgetarrowoptions{) new}<0pt%
    \pgfutil@tempdima=2pt%
    \advance\pgfutil@tempdima by1.5\pgflinewidth%
    \pgfutil@tempdimb=0.0625\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
    \pgfutil@tempdimb=0.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{) new}%
    \pgfutil@tempdima=0.28125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.21875\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.5\pgflinewidth}  
  \fi
}
{
  \ifdim\pgfgetarrowoptions{) new}<0pt%
    \pgfutil@tempdima=2pt%
    \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{) new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 2%
    \pgftransformxshift{-0.0625\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{.25\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{.25\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-.5\pgfutil@tempdima}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative round bracket reversed arrow
\pgfarrowsdeclarereversed{) new}{( new}{( new}{) new}

% alternative square bracket arrow. Use with {[ new}-{] new}
\pgfarrowsdeclare{[ new}{] new}
{
  \pgfutil@tempdima=1pt%
  \advance\pgfutil@tempdima by1.25\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdima}
  \pgfarrowsrightextend{+.5\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfutil@tempdimb=\pgfutil@tempdima%
  \advance\pgfutil@tempdimb by\pgflinewidth%
  \unless\ifdim\pgfgetarrowoptions{] new}<0pt%
    \pgfutil@tempdima=\pgfgetarrowoptions{] new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 2%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdimb}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-.5\pgfutil@tempdimb}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative square bracket reversed arrow. Use with {] new}-{[ new}
\pgfarrowsdeclarereversed{] new}{[ new}{[ new}{] new}

% alternative | arrow
\pgfarrowsdeclare{| new}{| new}
{
  \pgfarrowsleftextend{+-0.25\pgflinewidth}
  \pgfarrowsrightextend{+.75\pgflinewidth}
}
{
  \ifdim\pgfgetarrowoptions{| new}<0pt%
    \pgfutil@tempdima=2pt%
    \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{| new}%
    \advance\pgfutil@tempdima by -\pgflinewidth% due to rect line cap
    \divide\pgfutil@tempdima by 2%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetrectcap
  \pgfpathmoveto{\pgfqpoint{0.25\pgflinewidth}{-\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.25\pgflinewidth}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative angle 45 arrow
\pgfarrowsdeclare{angle 45 new}{angle 45 new}
{
  \ifdim\pgfgetarrowoptions{angle 45 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=8.705\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by1.28\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 45 new}%
    \advance\pgfutil@tempdima by -1.30656\pgflinewidth% 0.5*cosec(\alpha/2)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+1.30656\pgflinewidth}  
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{angle 45 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 45 new}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)} 
    \pgfpathmoveto{\pgfqpointpolar{157.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-157.5}{\pgfutil@tempdima}}
    \pgfusepathqstroke
  \fi
}

% alternative angle 45 reversed arrow
\pgfarrowsdeclarereversed{angle 45 new reversed}{angle 45 new reversed}{angle 45 new}{angle 45 new}

% alternative angle 60 arrow
\pgfarrowsdeclare{angle 60 new}{angle 60 new}
{
  \ifdim\pgfgetarrowoptions{angle 60 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=7.29\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 60 new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgflinewidth}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{angle 60 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 60 new}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}    
    \pgfpathmoveto{\pgfqpointpolar{150}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-150}{\pgfutil@tempdima}}
    \pgfusepathqstroke
  \fi
}

% alternative angle 60 reversed arrow
\pgfarrowsdeclarereversed{angle 60 new reversed}{angle 60 new reversed}{angle 60 new}{angle 60 new}

% alternative angle 90 arrow
\pgfarrowsdeclare{angle 90 new}{angle 90 new}
{
  \ifdim\pgfgetarrowoptions{angle 90 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=5.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.707\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 90 new}%
    \advance\pgfutil@tempdima by -0.70711\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.70711\pgflinewidth}  
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{angle 90 new}<0pt%
    \pgfutil@tempdima=0.3pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{angle 90 new}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)
    \pgfpathmoveto{\pgfqpoint{-\pgfutil@tempdima}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}
    \pgfusepathqstroke
  \fi    
}

% alternative angle 90 reversed arrow
\pgfarrowsdeclarereversed{angle 90 new reversed}{angle 90 new reversed}{angle 90 new}{angle 90 new}

% original butt cap arrow (just for completeness)
\pgfarrowsdeclare{butt cap new}{butt cap new}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+.5\pgflinewidth}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}

% alternative diamond arrow
\pgfarrowsdeclare{diamond new}{diamond new}
{
  \ifdim\pgfgetarrowoptions{diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \pgfutil@tempdimb=13\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=1\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{diamond new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsleftextend{+-0.5\pgflinewidth}% due to the round cap
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{diamond new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 14%
    \pgftransformxshift{13\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{1\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

% original fast cap arrow (just for completeness)
\pgfarrowsdeclare{fast cap new}{fast cap new}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+2\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}

% original fast cap reversed arrow (just for completeness)
\pgfarrowsdeclare{fast cap new reversed}{fast cap new reversed}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+2\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}

% alternative hooks arrow
\pgfarrowsdeclare{hooks new}{hooks new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{hooks new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{hooks new}%
    \pgfutil@tempdima=0.3125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.1875\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}%
  \fi
}
{
  \ifdim\pgfgetarrowoptions{hooks new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{hooks new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 12%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathmoveto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

% alternative hooks reversed arrow
\pgfarrowsdeclarereversed{hooks new reversed}{hooks new reversed}{hooks new}{hooks new}

% original implies arrow (just for completeness)
\pgfarrowsdeclare{implies new}{implies new}
{
  \pgfmathsetlength{\pgfutil@tempdima}{.25\pgflinewidth+.25*\pgfinnerlinewidth}%
  \pgfmathsetlength{\pgfutil@tempdimb}{.5\pgflinewidth-.5*\pgfinnerlinewidth}%
  \pgfarrowsrightextend{2\pgfutil@tempdima+.5\pgfutil@tempdimb}
  \pgfarrowsleftextend{1.3\pgfutil@tempdima+.5\pgfutil@tempdimb}
}
{
  \pgfmathsetlength{\pgfutil@tempdima}{.25\pgflinewidth+.25*\pgfinnerlinewidth}%
  \pgfmathsetlength{\pgfutil@tempdimb}{.5\pgflinewidth-.5*\pgfinnerlinewidth}%
  \pgfsetlinewidth{\pgfutil@tempdimb}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-1.4\pgfutil@tempdima}{2.65\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfpoint{-0.75\pgfutil@tempdima}{1.25\pgfutil@tempdima}}
  {\pgfpoint{1\pgfutil@tempdima}{0.05\pgfutil@tempdima}}
  {\pgfpoint{2\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{1\pgfutil@tempdima}{-0.05\pgfutil@tempdima}}
  {\pgfpoint{-.75\pgfutil@tempdima}{-1.25\pgfutil@tempdima}}
  {\pgfpoint{-1.4\pgfutil@tempdima}{-2.65\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative latex arrow
\pgfarrowsdeclare{latex new}{latex new}
{
  \ifdim\pgfgetarrowoptions{latex new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
    \pgfarrowsleftextend{+-1\pgfutil@tempdima}
    \pgfarrowsrightextend{+9\pgfutil@tempdima}
  \else
     \pgfutil@tempdima=\pgfgetarrowoptions{latex new}%
     \advance\pgfutil@tempdima by -0.5pt% to minimize the arrow shaft
     \pgfarrowsleftextend{+-0.5pt}
     \pgfarrowsrightextend{\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{latex new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{latex new}%
    \divide\pgfutil@tempdima by 10%
    \pgfutil@tempdimb=\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.5pt%
    \pgftransformxshift{\pgfutil@tempdimb}% to minimize the arrow shaft
  \fi
  \pgfpathmoveto{\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{6.3333\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{2\pgfutil@tempdima}{2\pgfutil@tempdima}}
    {\pgfqpoint{-1\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-1\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2\pgfutil@tempdima}{-2\pgfutil@tempdima}}
    {\pgfqpoint{6.3333\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfusepathqfill
}

% alternative latex reversed arrow
\pgfarrowsdeclarereversed{latex new reversed}{latex new reversed}{latex new}{latex new}

% alternative latex' arrow
\pgfarrowsdeclare{latex' new}{latex' new}
{
  \ifdim\pgfgetarrowoptions{latex' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfarrowsleftextend{+-4\pgfutil@tempdima}
    \pgfarrowsrightextend{+6\pgfutil@tempdima}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{latex' new}%
    \pgfutil@tempdimb=0.8125\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.5pt%
    \advance\pgfutil@tempdima by -\pgfutil@tempdimb%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}% to minimize the arrow shaft
    \pgfarrowsrightextend{+\pgfutil@tempdimb}%
  \fi
}
{
  \ifdim\pgfgetarrowoptions{latex' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{latex' new}%
    \divide\pgfutil@tempdima by 10%
    \pgfutil@tempdimb=2.125\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.5pt%
    \pgftransformxshift{\pgfutil@tempdimb}% to minimize the arrow shaft
  \fi
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-1\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
    {\pgfqpoint{-4\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-1.5\pgfutil@tempdima}{1\pgfutil@tempdima}}
    {\pgfqpoint{-1.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
    {\pgfqpoint{-4\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-1\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
    {\pgfqpoint{3.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfusepathqfill
}

% alternative latex' reversed arrow
\pgfarrowsdeclarereversed{latex' new reversed}{latex' new reversed}{latex' new}{latex' new}

% alternative left hook arrow
\pgfarrowsdeclare{left hook new}{left hook new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{left hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left hook new}%
    \pgfutil@tempdima=0.3125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.1875\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{left hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left hook new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 12%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

% alternative left hook reversed arrow
\pgfarrowsdeclarereversed{left hook new reversed}{left hook new reversed}{left hook new}{left hook new}

% alternative left to arrow
\pgfarrowsdeclare{left to new}{left to new}
{
  \ifdim\pgfgetarrowoptions{left to new}<0pt%
    \pgfutil@tempdima=-0.84pt%
    \advance\pgfutil@tempdima by-1.3\pgflinewidth%
    \pgfutil@tempdimb=0.21pt%
    \advance\pgfutil@tempdimb by.625\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.8\pgflinewidth}%
  \fi
}
{
  \ifdim\pgfgetarrowoptions{left to new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfutil@tempdimb=0pt%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{-\pgfutil@tempdimb}
  \fi  
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{0.55\pgfutil@tempdima}{-0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}} 
  \pgfpathlineto{\pgfqpoint{\pgfutil@tempdimb}{-0.125\pgflinewidth}}
  \pgfusepathqstroke
}

% alternative left to reversed arrow
\pgfarrowsdeclare{left to new reversed}{left to new reversed}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \ifdim\pgfgetarrowoptions{left to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth% 
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.9\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new reversed}%
    \advance\pgfutil@tempdima by 0.1\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{left to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{-0.125\pgflinewidth}}
  }
  \pgfusepathqstroke
}

% alternative o arrow
\pgfarrowsdeclare{o new}{o new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{o new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=9\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{o new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{ 
  \ifdim\pgfgetarrowoptions{o new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{o new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 9%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfpathcircle{\pgfqpoint{4.5\pgfutil@tempdima}{0pt}}{4.5\pgfutil@tempdima}%
  \pgfusepathqstroke
}

% alternative open diamond arrow
\pgfarrowsdeclare{open diamond new}{open diamond new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}% due to the round cap
  \ifdim\pgfgetarrowoptions{open diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \pgfutil@tempdimb=14\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open diamond new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{open diamond new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open diamond new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 14%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{14\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}

% alternative open square arrow
\pgfarrowsdeclare{open square new}{open square new}
{
  \ifdim\pgfgetarrowoptions{open square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \advance\pgfutil@tempdima by7\pgfutil@tempdima%
    \advance\pgfutil@tempdima by.5\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open square new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
  \fi
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfarrowsrightextend{+\pgfutil@tempdima}
}
{
  \ifdim\pgfgetarrowoptions{open square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open square new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 8%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{8\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{8\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}

% alternative open triangle 45 arrow
\pgfarrowsdeclare{open triangle 45 new}{open triangle 45 new}
{
  \ifdim\pgfgetarrowoptions{open triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=9.205\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 45 new}%
    \advance\pgfutil@tempdimb by -0.5\pgflinewidth%
  \fi
    \pgfarrowsleftextend{+-.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin  
  \ifdim\pgfgetarrowoptions{open triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 45 new}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)}    
    \pgfpathmoveto{\pgfqpointpolar{157.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-157.5}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi    
}

% alternative open triangle 45 reversed arrow
\pgfarrowsdeclare{open triangle 45 new reversed}{open triangle 45 new reversed}
{
  \ifdim\pgfgetarrowoptions{open triangle 45 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfarrowsleftextend{+-1.28\pgflinewidth}
    \pgfutil@tempdimb=9.205\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \else
    \pgfarrowsleftextend{+-1.30656\pgflinewidth}%
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 45 new reversed}%
    \advance\pgfutil@tempdimb by -1.30656\pgflinewidth%
  \fi
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 45 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpointpolar{23}{10\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-23}{10\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 45 new reversed}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)}    
    \pgfpathmoveto{\pgfqpointpolar{22.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-22.5}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi  
}

% alternative open triangle 60 arrow
\pgfarrowsdeclare{open triangle 60 new}{open triangle 60 new}
{
  \ifdim\pgfgetarrowoptions{open triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=7.794\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 60 new}%
    \advance\pgfutil@tempdimb by -0.5\pgflinewidth%
  \fi
    \pgfarrowsleftextend{+-.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 60 new}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}  
    \pgfpathmoveto{\pgfqpointpolar{150}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-150}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi    
}

% alternative open triangle 60 reversed
\pgfarrowsdeclare{open triangle 60 new reversed}{open triangle 60 new reversed}
{
  \ifdim\pgfgetarrowoptions{open triangle 60 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%   
    \pgfutil@tempdimb=7.794\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth% 
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 60 new reversed}%
    \advance\pgfutil@tempdimb by -\pgflinewidth%
  \fi
  \pgfarrowsleftextend{+-\pgflinewidth}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 60 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%  
    \pgfpathmoveto{\pgfqpointpolar{30}{9\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-30}{9\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 60 new reversed}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}    
    \pgfpathmoveto{\pgfqpointpolar{30}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-30}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi  
}

% alternative open triangle 90 arrow
\pgfarrowsdeclare{open triangle 90 new}{open triangle 90 new}
{
  \ifdim\pgfgetarrowoptions{open triangle 90 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=6\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 90 new}%
    \advance\pgfutil@tempdimb by -0.5\pgflinewidth%
  \fi
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 90 new}<0pt%  
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth% 
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 90 new}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)  
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi    
}

% alternative open triangle 90 reversed arrow
\pgfarrowsdeclare{open triangle 90 new reversed}{open triangle 90 new reversed}
{
  \ifdim\pgfgetarrowoptions{open triangle 90 new reversed}<0pt%  
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfarrowsleftextend{+-.707\pgflinewidth}
    \pgfutil@tempdimb=6\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdimb=\pgfgetarrowoptions{open triangle 90 new reversed}%
    \advance\pgfutil@tempdimb by -0.70711\pgflinewidth%
    \pgfarrowsleftextend{+-0.70711\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{open triangle 90 new reversed}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
   \else
    \pgfutil@tempdima=\pgfgetarrowoptions{open triangle 90 new reversed}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)   
    \pgfpathmoveto{\pgfqpoint{\pgfutil@tempdima}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqstroke
  \fi  
}

% alternative right hook arrow
\pgfarrowsdeclare{right hook new}{right hook new}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \ifdim\pgfgetarrowoptions{right hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right hook new}%
    \pgfutil@tempdima=0.3125\pgfutil@tempdima%
    \advance\pgfutil@tempdima by 0.1875\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{right hook new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.2\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right hook new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 12%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}
    {\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}
    {\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative right hook reversed arrow
\pgfarrowsdeclarereversed{right hook new reversed}{right hook new reversed}{right hook new}{right hook new}

% alternative right to arrow
\pgfarrowsdeclare{right to new}{right to new}
{
  \ifdim\pgfgetarrowoptions{right to new}<0pt%
    \pgfutil@tempdima=-0.84pt%
    \advance\pgfutil@tempdima by-1.3\pgflinewidth%
    \pgfutil@tempdimb=0.21pt%
    \advance\pgfutil@tempdimb by.625\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.8\pgflinewidth}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{right to new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfutil@tempdimb=0pt%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{left to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{-\pgfutil@tempdimb}
  \fi  
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{0.55\pgfutil@tempdima}{0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{\pgfutil@tempdimb}{0.125\pgflinewidth}}
  \pgfusepathqstroke
}

% alternative right to reversed arrow
\pgfarrowsdeclare{right to new reversed}{right to new reversed}
{
 \pgfarrowsleftextend{+-.1\pgflinewidth}
  \ifdim\pgfgetarrowoptions{right to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth% 
    \pgfutil@tempdimb=3.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.9\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right to new reversed}%
    \advance\pgfutil@tempdima by 0.1\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{right to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{right to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth 
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap 
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{-0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto
      {\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
      {\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
      {\pgfqpoint{0pt}{0.125\pgflinewidth}}
  }
  \pgfusepathqstroke
}

% original round cap arrow (just for completeness)
\pgfarrowsdeclare{round cap new}{round cap new}
{
  \pgfarrowsleftextend{+0pt}
  \pgfarrowsrightextend{+\pgflinewidth}
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}

% original serif cm arrow (just for completeness)
\pgfarrowsdeclare{serif cm new}{serif cm new}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgfarrowsleftextend{+-.75\pgfutil@tempdima}
  \pgfarrowsrightextend{+.04\pgflinewidth}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgftransformxshift{.04\pgflinewidth}
  \pgfpathmoveto{\pgfqpoint{-.75\pgfutil@tempdima}{.5\pgflinewidth}}
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{.5\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{1.95\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{1.95\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.04\pgflinewidth}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-.04\pgflinewidth}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{-1.95\pgfutil@tempdima}}  
  \pgfpathlineto{\pgfqpoint{-.375\pgfutil@tempdima}{-1.95\pgfutil@tempdima}}  
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.5\pgflinewidth}}
    {\pgfqpoint{-.75\pgfutil@tempdima}{-.5\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}

% original space arrow (just for completeness)
\pgfarrowsdeclare{space new}{space new}
{
  \pgfutil@tempdima=0.88pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{0pt}
  \pgfarrowsrightextend{\pgfutil@tempdima}
}
{}

% alternative square arrow
\pgfarrowsdeclare{square new}{square new}
{
  \ifdim\pgfgetarrowoptions{square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \advance\pgfutil@tempdima by.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{square new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsleftextend{+-.5\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{square new}<0pt%
    \pgfutil@tempdima=0.4pt%
    \advance\pgfutil@tempdima by.275\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{square new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 8%
    \pgftransformxshift{7\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{1\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-7\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-7\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{1\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

% alternative stealth arrow
\pgfarrowsdeclare{stealth new}{stealth new}
{
  \ifdim\pgfgetarrowoptions{stealth new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth new}%
    \divide\pgfutil@tempdima by 8%
  \fi
  \pgfarrowsleftextend{+-3\pgfutil@tempdima}
  \pgfarrowsrightextend{+5\pgfutil@tempdima}
}
{
  \ifdim\pgfgetarrowoptions{stealth new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \pgfutil@tempdimb=\pgflinewidth%
    \ifdim\pgfinnerlinewidth>0pt%
      \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
    \fi
    \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth new}%
    \divide\pgfutil@tempdima by 8%
  \fi
  \pgfpathmoveto{\pgfqpoint{5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqfill
}

% alternative stealth reversed arrow
\pgfarrowsdeclarereversed{stealth new reversed}{stealth new reversed}{stealth new}{stealth new}

% alternative stealth' arrow
\pgfarrowsdeclare{stealth' new}{stealth' new}
{
  \ifdim\pgfgetarrowoptions{stealth' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
    \pgfutil@tempdimb=6\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=2\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth' new}%
    \pgfutil@tempdimb=0.71875\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.21875\pgflinewidth%
    \advance\pgfutil@tempdima by -\pgfutil@tempdimb%
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \fi  
}
{
  \ifdim\pgfgetarrowoptions{stealth' new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{stealth' new}%
    \advance\pgfutil@tempdima by -\pgflinewidth%
    \divide\pgfutil@tempdima by 8%
    \pgftransformxshift{3.75\pgfutil@tempdima}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-3\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
    {\pgfqpoint{-6\pgfutil@tempdima}{3.25\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-3\pgfutil@tempdima}{1\pgfutil@tempdima}}
    {\pgfqpoint{-3\pgfutil@tempdima}{-1\pgfutil@tempdima}}
    {\pgfqpoint{-6\pgfutil@tempdima}{-3.25\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-3\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
    {\pgfqpoint{-.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

% alternative stealth' reversed arrow
\pgfarrowsdeclarereversed{stealth' new reversed}{stealth' new reversed}{stealth' new}{stealth' new}

% alternative to arrow
\pgfarrowsdeclare{to new}{to new}
{
  \ifdim\pgfgetarrowoptions{to new}<0pt%
    \pgfutil@tempdima=-0.84pt%
    \advance\pgfutil@tempdima by-1.3\pgflinewidth%
    \pgfutil@tempdimb=0.21pt%
    \advance\pgfutil@tempdimb by.625\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-\pgfutil@tempdima}
    \pgfarrowsrightextend{+0.8\pgflinewidth}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{to new}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.75\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{-\pgfutil@tempdimb}
  \fi
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
    {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
    {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
    {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
    {\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative to reversed arrow
\pgfarrowsdeclare{to new reversed}{to new reversed}
{
  \ifdim\pgfgetarrowoptions{to new reversed}<0pt%
    \pgfutil@tempdima=-0.21pt%
    \advance\pgfutil@tempdima by-0.475\pgflinewidth%
    \pgfutil@tempdimb=0.98pt%
    \advance\pgfutil@tempdimb by1.45\pgflinewidth%
    \pgfarrowsleftextend{+\pgfutil@tempdima}
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% arbitrary value (2*0.5*0.8\pgflinewidth)
    \pgfarrowsleftextend{+-0.8\pgflinewidth}
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \ifdim\pgfgetarrowoptions{to new reversed}<0pt%
    \pgfutil@tempdima=0.28pt%
    \advance\pgfutil@tempdima by.3\pgflinewidth%
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{to new reversed}%
    \advance\pgfutil@tempdima by -0.8\pgflinewidth% because thickness is set to 0.8\pgflinewidth
    \divide\pgfutil@tempdima by 15%    
    \multiply\pgfutil@tempdima by 4%
    \pgfutil@tempdimb=0.25\pgfutil@tempdima%  
    \advance\pgfutil@tempdimb by -0.4\pgflinewidth% arbitrary value (0.5*0.8\pgflinewidth)
    \pgftransformxshift{\pgfutil@tempdimb}
  \fi
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfsetlinewidth{+0.8\pgflinewidth}
  \pgfpathmoveto{\pgfqpoint{3.5\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{3.25\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
    {\pgfqpoint{0.5\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
    {\pgfqpoint{-0.25\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{0.5\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
    {\pgfqpoint{3.25\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
    {\pgfqpoint{3.5\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}

% alternative triangle 45 arrow
\pgfarrowsdeclare{triangle 45 new}{triangle 45 new}
{
  \ifdim\pgfgetarrowoptions{triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=8.705\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by1.28\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 45 new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%   
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{triangle 45 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                  {\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 45 new}%
    \advance\pgfutil@tempdima by -1.80656\pgflinewidth% -(1.30656+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(22.5)}    
    \pgfpathmoveto{\pgfqpointpolar{157.5}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-157.5}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \fi
}

% alternative triangle 45 reversed arrow
\pgfarrowsdeclarereversed{triangle 45 new reversed}{triangle 45 new reversed}{triangle 45 new}{triangle 45 new}

% alternative triangle 60 arrow
\pgfarrowsdeclare{triangle 60 new}{triangle 60 new}
{
  \ifdim\pgfgetarrowoptions{triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=7.29\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 60 new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%   
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{triangle 60 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%   
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
                               {\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 60 new}%
    \advance\pgfutil@tempdima by -1.5\pgflinewidth% -(1+0.5)
    \pgftransformxshift{\pgfutil@tempdima}
    \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(30)}    
    \pgfpathmoveto{\pgfqpointpolar{150}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfpointorigin}
    \pgfpathlineto{\pgfqpointpolar{-150}{\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \fi
}

% alternative triangle 60 reversed arrow
\pgfarrowsdeclarereversed{triangle 60 new reversed}{triangle 60 new reversed}{triangle 60 new}{triangle 60 new}

% alternative triangle 90 arrow
\pgfarrowsdeclare{triangle 90 new}{triangle 90 new}
{
  \ifdim\pgfgetarrowoptions{triangle 90 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfutil@tempdimb=5.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by.5\pgflinewidth%
    \pgfarrowsleftextend{+-\pgfutil@tempdimb}
    \pgfutil@tempdimb=.5\pgfutil@tempdima%
    \advance\pgfutil@tempdimb by0.707\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \else
    \pgfarrowsleftextend{+-0.5\pgflinewidth}
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 90 new}%
    \advance\pgfutil@tempdima by -0.5\pgflinewidth%
    \pgfarrowsrightextend{+\pgfutil@tempdima}
  \fi
}
{
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \ifdim\pgfgetarrowoptions{triangle 90 new}<0pt%
    \pgfutil@tempdima=0.5pt%
    \advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \else
    \pgfutil@tempdima=\pgfgetarrowoptions{triangle 90 new}%
    \advance\pgfutil@tempdima by -1.20711\pgflinewidth% -(0.70711+0.5)
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
    \pgfpathlineto{\pgfqpoint{\pgfutil@tempdima}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfutil@tempdima}}
    \pgfpathclose
    \pgfusepathqfillstroke
  \fi
}

% alternative triangle 90 reversed arrow
\pgfarrowsdeclarereversed{triangle 90 new reversed}{triangle 90 new reversed}{triangle 90 new}{triangle 90 new}

% original triangle 90 cap arrow (just for completeness)
\pgfarrowsdeclare{triangle 90 cap new}{triangle 90 cap new}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfusepathqfill
}

% original triangle 90 cap reversed arrow (just for completeness)
\pgfarrowsdeclare{triangle 90 cap new reversed}{triangle 90 cap new reversed}
{
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfarrowsrightextend{+\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0\pgflinewidth}}
  \pgfusepathqfill
}

% alias alternative to arrow
\pgfarrowsdeclarealias{< new}{> new}{to new}{to new}

% alias alternative to reversed arrow
\pgfarrowsdeclarealias{> new}{< new}{to new reversed}{to new reversed}

% arrow head length code
\pgfsetarrowoptions{* new}{-1pt}
\pgfsetarrowoptions{< new}{-1pt}
\pgfsetarrowoptions{> new}{-1pt}
\pgfsetarrowoptions{) new}{-1pt}
\pgfsetarrowoptions{( new}{-1pt}
\pgfsetarrowoptions{[ new}{-1pt}
\pgfsetarrowoptions{] new}{-1pt}
\pgfsetarrowoptions{| new}{-1pt}
\pgfsetarrowoptions{angle 45 new}{-1pt}
\pgfsetarrowoptions{angle 45 new reversed}{-1pt}
\pgfsetarrowoptions{angle 60 new}{-1pt}
\pgfsetarrowoptions{angle 60 new reversed}{-1pt}
\pgfsetarrowoptions{angle 90 new}{-1pt}
\pgfsetarrowoptions{angle 90 new reversed}{-1pt}
\pgfsetarrowoptions{diamond new}{-1pt}
\pgfsetarrowoptions{hooks new}{-1pt}
\pgfsetarrowoptions{hooks new reversed}{-1pt}
\pgfsetarrowoptions{latex new}{-1pt}
\pgfsetarrowoptions{latex new reversed}{-1pt}
\pgfsetarrowoptions{latex' new}{-1pt}
\pgfsetarrowoptions{latex' new reversed}{-1pt}
\pgfsetarrowoptions{left hook new}{-1pt}
\pgfsetarrowoptions{left hook new reversed}{-1pt}
\pgfsetarrowoptions{left to new}{-1pt}
\pgfsetarrowoptions{left to new reversed}{-1pt}
\pgfsetarrowoptions{o new}{-1pt}
\pgfsetarrowoptions{open diamond new}{-1pt}
\pgfsetarrowoptions{open square new}{-1pt}
\pgfsetarrowoptions{open triangle 45 new}{-1pt}
\pgfsetarrowoptions{open triangle 45 new reversed}{-1pt}
\pgfsetarrowoptions{open triangle 60 new}{-1pt}
\pgfsetarrowoptions{open triangle 60 new reversed}{-1pt}
\pgfsetarrowoptions{open triangle 90 new}{-1pt}
\pgfsetarrowoptions{open triangle 90 new reversed}{-1pt}
\pgfsetarrowoptions{right hook new}{-1pt}
\pgfsetarrowoptions{right hook new reversed}{-1pt}
\pgfsetarrowoptions{right to new}{-1pt}
\pgfsetarrowoptions{right to new reversed}{-1pt}
\pgfsetarrowoptions{square new}{-1pt}
\pgfsetarrowoptions{stealth new}{-1pt}
\pgfsetarrowoptions{stealth new reversed}{-1pt}
\pgfsetarrowoptions{stealth' new}{-1pt}
\pgfsetarrowoptions{stealth' new reversed}{-1pt}
\pgfsetarrowoptions{to new}{-1pt}
\pgfsetarrowoptions{to new reversed}{-1pt}
\pgfsetarrowoptions{triangle 45 new}{-1pt}
\pgfsetarrowoptions{triangle 45 new reversed}{-1pt}
\pgfsetarrowoptions{triangle 60 new}{-1pt}
\pgfsetarrowoptions{triangle 60 new reversed}{-1pt}
\pgfsetarrowoptions{triangle 90 new}{-1pt}
\pgfsetarrowoptions{triangle 90 new reversed}{-1pt}

\pgfkeys{/tikz/.cd, arrow head/.default=-1pt, arrow head/.code={%
  \pgfsetarrowoptions{* new}{#1}%
  \pgfsetarrowoptions{< new}{#1}%
  \pgfsetarrowoptions{> new}{#1}%
  \pgfsetarrowoptions{) new}{#1}%
  \pgfsetarrowoptions{( new}{#1}%
  \pgfsetarrowoptions{[ new}{#1}%
  \pgfsetarrowoptions{] new}{#1}%
  \pgfsetarrowoptions{| new}{#1}%
  \pgfsetarrowoptions{angle 45 new}{#1}%
  \pgfsetarrowoptions{angle 45 new reversed}{#1}%
  \pgfsetarrowoptions{angle 60 new}{#1}%
  \pgfsetarrowoptions{angle 60 new reversed}{#1}%
  \pgfsetarrowoptions{angle 90 new}{#1}%
  \pgfsetarrowoptions{angle 90 new reversed}{#1}%
  \pgfsetarrowoptions{diamond new}{#1}%
  \pgfsetarrowoptions{hooks new}{#1}%
  \pgfsetarrowoptions{hooks new reversed}{#1}%
  \pgfsetarrowoptions{latex new}{#1}%
  \pgfsetarrowoptions{latex new reversed}{#1}%
  \pgfsetarrowoptions{latex' new}{#1}%
  \pgfsetarrowoptions{latex' new reversed}{#1}%
  \pgfsetarrowoptions{left hook new}{#1}%
  \pgfsetarrowoptions{left hook new reversed}{#1}%
  \pgfsetarrowoptions{left to new}{#1}%
  \pgfsetarrowoptions{left to new reversed}{#1}%
  \pgfsetarrowoptions{o new}{#1}%
  \pgfsetarrowoptions{open diamond new}{#1}%
  \pgfsetarrowoptions{open square new}{#1}%
  \pgfsetarrowoptions{open triangle 45 new}{#1}%
  \pgfsetarrowoptions{open triangle 45 new reversed}{#1}%
  \pgfsetarrowoptions{open triangle 60 new}{#1}%
  \pgfsetarrowoptions{open triangle 60 new reversed}{#1}%
  \pgfsetarrowoptions{open triangle 90 new}{#1}%
  \pgfsetarrowoptions{open triangle 90 new reversed}{#1}%
  \pgfsetarrowoptions{right hook new}{#1}%
  \pgfsetarrowoptions{right hook new reversed}{#1}%
  \pgfsetarrowoptions{right to new}{#1}%
  \pgfsetarrowoptions{right to new reversed}{#1}%
  \pgfsetarrowoptions{square new}{#1}%
  \pgfsetarrowoptions{stealth new}{#1}%
  \pgfsetarrowoptions{stealth new reversed}{#1}%
  \pgfsetarrowoptions{stealth' new}{#1}%
  \pgfsetarrowoptions{stealth' new reversed}{#1}%
  \pgfsetarrowoptions{to new}{#1}%
  \pgfsetarrowoptions{to new reversed}{#1}%
  \pgfsetarrowoptions{triangle 45 new}{#1}%
  \pgfsetarrowoptions{triangle 45 new reversed}{#1}%
  \pgfsetarrowoptions{triangle 60 new}{#1}%
  \pgfsetarrowoptions{triangle 60 new reversed}{#1}%
  \pgfsetarrowoptions{triangle 90 new}{#1}%
  \pgfsetarrowoptions{triangle 90 new reversed}{#1}%
}}

\endinput

==> tikzlibraryarrows.new.code.tex <==
\usepgflibrary{arrows.new}

\endinput
